Uncovering Social Network Sybils in the Wild

Sybil accounts are fake identities created to unfairly increase the power or resources of a single malicious user. Researchers have long known about the existence of Sybil accounts in online communities such as file-sharing systems, but have not been able to perform large scale measurements to detect them or measure their activities. In this paper, we describe our efforts to detect, characterize and understand Sybil account activity in the Renren online social network (OSN). We use ground truth provided by Renren Inc. to build measurement based Sybil account detectors, and deploy them on Renren to detect over 100,000 Sybil accounts. We study these Sybil accounts, as well as an additional 560,000 Sybil accounts caught by Renren, and analyze their link creation behavior. Most interestingly, we find that contrary to prior conjecture, Sybil accounts in OSNs do not form tight-knit communities. Instead, they integrate into the social graph just like normal users. Using link creation timestamps, we verify that the large majority of links between Sybil accounts are created accidentally, unbeknownst to the attacker. Overall, only a very small portion of Sybil accounts are connected to other Sybils with social links. Our study shows that existing Sybil defenses are unlikely to succeed in today's OSNs, and we must design new techniques to effectively detect and defend against Sybil attacks.

==> background.tex <==
\section{Related Work}
\label{sec:background}

\para{OSN Spam.} Recent studies have characterized the growing OSN spam
problem on Facebook~\cite{osnspam-imc10} and
Twitter~\cite{twitterspam-ccs10}. These studies rely on offline heuristics
to identify spam content in status updates/tweets, as well as aberrant
behavior that is indicative of spamming. The authors locate millions of spam
messages on each OSN, and use them to analyze the large scale, coordinated
spam campaigns. In contrast, our study is focused
on the graph topological characteristics of malicious accounts, rather than
spam content.

\para{OSN Spam Detection.} Various techniques borrowed from e-mail spam
detection have been applied to OSN spam. Webb et. al. use
honeypot accounts on MySpace to trap spammers who attempt to friend
them~\cite{webb_socialhoneypots}. Our results indicate that unless social
honeypots are engineered to appear popular, they are unlikely to be
targeted by spammers.

Other studies have leveraged Bayesian filters and SVMs to identify spammers on
Twitter~\cite{yardi-detecting-spam,twitterspam-ceas10,twitterspam-secrypt10}
and Facebook~\cite{osnspam-acsac10}. These techniques work well on Twitter,
since Sybil friending behavior can be identified using publicly available following
and followed information. However, detection on OSNs like Facebook and Renren is
less successful, since the only publicly available indicators are laggy. Our
Sybil detector overcomes this issue by leveraging friend invitation information
that is only accessible from within Renren.

%
%Although each of
%these algorithms is implemented slightly differently, it has been shown that they
%all generalize to the detection of densely connection communities of Sybils within the
%social graph~\cite{sybilroundup-sigcom10}.
%
%The assumption that Sybils on OSNs form clusters is based on intuitive notions of
%Sybil behavior and goals. It is assumed that attackers want to integrate Sybils into
%the general population, but they are unable to do so reliably because users are reluctant
%to become friends with unknown, suspicious users. Thus, Sybils first friend each other
%in order to make themselves appear more legitimate, before attempting to friend normal
%users. However, because the number of edges between Sybils is larger than the number of
%edges to honest users, Sybils end up coallescing into clusters.
%
%However, it has never been demonstrated that any of these assumptions are true on
%today's OSNs. Specifically: do Sybils form edges between themselves, and does this
%lead to identifiable clusters? How likely are users to accept friend requests from Sybils?
%Do different types of users (popular/unpopular, male/female, \etc) respond differently to
%friend requests from Sybils, if so how, and is this behavior exploited by attackers?


==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper we make two contributions to the area of Sybil
detection on OSNs. First, we use ground-truth data about the
behavior of Sybils in the wild to create a measurement-based,
real-time Sybil detector. We show that a computationally
efficient, threshold-based classifier is sufficient to catch
99\% of Sybils, with low false positive and negative rates.
We have deployed our detector on Renren's production systems,
and to date it has led to the identification and banning
of over 100,000 Sybil accounts.

Our second contribution is a first-of-its-kind characterization
of Sybil graph topology on a major OSN. Using edge creation
information for
660,000 Sybil accounts on Renren, we show that Sybils in the wild
do not obey behavioral assumptions that underlie previous work
on decentralized Sybil detectors. Specifically, we demonstrate
that the vast majority (80\%) of Sybils do not connect to other
Sybils. Even in cases where Sybils do form connected components,
these clusters are loose, rather than tightly knit. Temporal
analysis indicates that these Sybil edges are formed accidentally,
rather than intentionally by attackers. These findings
suggest that new approaches are needed to perform
decentralized detection of Sybil accounts on OSNs. 
